Brain Imaging Foundation Models, Are We There Yet? A Systematic Review of Foundation Models for Brain Imaging and Biomedical Research

Foundation models (FMs), large neural networks pretrained on extensive and diverse datasets, have revolutionized artificial intelligence and shown significant promise in medical imaging by enabling robust performance with limited labeled data. Although numerous surveys have reviewed the application of FM in healthcare care, brain imaging remains underrepresented, despite its critical role in the diagnosis and treatment of neurological diseases using modalities such as MRI, CT, and PET. Existing reviews either marginalize brain imaging or lack depth on the unique challenges and requirements of FM in this domain, such as multimodal data integration, support for diverse clinical tasks, and handling of heterogeneous, fragmented datasets. To address this gap, we present the first comprehensive and curated review of FMs for brain imaging. We systematically analyze 161 brain imaging datasets and 86 FM architectures, providing information on key design choices, training paradigms, and optimizations driving recent advances. Our review highlights the leading models for various brain imaging tasks, summarizes their innovations, and critically examines current limitations and blind spots in the literature. We conclude by outlining future research directions to advance FM applications in brain imaging, with the aim of fostering progress in both clinical and research settings.

==> pages/background.tex <==
\section{Related work}
\label{sec-related_work}

%Present some existing surveys, their limitations, and how we are better.

With the increasing popularity of FMs, dozens of surveys have covered their application in healthcare \cite{moor2023foundation,azad_foundational_2023,qiu2023large,thirunavukarasu2023large,he_foundation_2024,shrestha2023medical,wang2023pretrained,zhou2023survey,yuan2023large,lee2024foundation,li2024progress,liu2024large,qiu2023pretraining,wang2023accelerating,zhang2024challenges,zhang2024datacentric,zhang_segment_2024,zhao_clip_2024,shi_survey_2024,he2023survey}. However, none of them focused on brain FMs, leading to a large disregard for the models tackling this critical field. For example, \citep{he_foundation_2024}, one of the largest reviews included 200 technical papers, but only 32 covered brain FMs; Similarly, the study of \citet{shi_survey_2024} provided one of the most thorough analysis and covered 76 research papers, but only ten tackled brain imaging. \citet{azad_foundational_2023}. Even surveys on specific family of FMs largely ignored FMs for brain imaging. The study from \citet{zhao_clip_2024}, the largest review of CLIP-based FMs, only covered seven brain FMs, while \citet{zhang_segment_2024} who explored SAM based FMs identified only nine brain FMs. 

We propose the first highly curated review of FMs dedicated to brain imaging, in which we uncovered and analyzed 86 models. 

Building effective deep learning models for brain imaging research is critical given the central role that imaging plays in managing brain diseases, from diagnosis and prognosis to treatment planning and follow-up of disease progression. Functional brain imaging also relies on specialized protocols and tracers  tailored to this organ, such as task-based and resting state fMRI or PET tracers targeting misfolded proteins in neuro-degenerative diseases for instance. 

Neurological disorders whose management benefits from brain imaging are quite diverse, including degenerative, vascular, and oncological disorders. Our study unveils the large imbalance in interest and efforts deployed to cover these pathologies in FMs research, despite the fact that some of these pathologies, being considered uncommon diseases (f.i. brain tumors), could be among those that benefit most from foundations models and their ability to perform in low amount of data settings. Indeed, FMs being trained on large diverse sets of data could handle rarer pathologies by leveraging knowledge from connex datasets. 


Given the importance of brain imaging, and the lack of any exhaustive survey on the field, our goal is to provide unique insights that are valuable to both the machine learning community and medical imaging users, contributing to bridge the gap between the two fields.
%Overall, we provide unique insights useful for both the machine learning community and medical imaging practitioners, and hope our research will contribute to bridge the gap between the two communities.   



==> pages/datasets_details.tex <==
\paragraph{Overview of datasets by impact}

We focused in the following on the five pathologies with the most datasets, glioma (both high and low grade, Fig.\ref{fig:dataset_glioma}), gliobastoma (Fig.\ref{fig:dataset_gbm}), metastasis (Fig.\ref{fig:dataset_metastasis}), Alzheimer (Fig.\ref{fig:dataset_alzheimer}), and Parkinson diseases (Fig.\ref{fig:dataset_parkinson}). Across all datastets, we notice that the largest datasets (biggest number of studies) are not necessary the most popular. The largest glioma dataset is BraTS23[], while the most cited is the Curious dataset[]. The largest GBM dataset is the UPenn-GBM dataset[], while the most cited is CGGA[]. The largest dataset for metastasis is the NYUMets while the the most popular is the UCSF-BMSR dataset. For both Parkinson and Alzehimer, the relevant dataset with the most citations and studies is the UKBioBank. It is worth nothing however that this dataset is a collection of a dozens of cohorts covering many organs and pathologies, and is a commercial (paid) dataset. For Alzheimer, combining the citations and studies across the 4 OASIS cohorts leads to a number of studies and citation of similar magnitude as the UKBioBank.  

It is also noteworthy that a few datasets with large number of studies have very few citations (MIRIAD, BrainAge, Rosmap, IvyGAP, ...). This could be due to the quality of the data, the ease of the data transfer/access, or the recent publication of the dataset.

\begin{Insight}[boxed title style={colback=pink}]
The largest brain datasets are not always the most popular in Cancer research. For neurogenerative diseases, while commercial datasets are popular, free public datasets are also accessible to foster imaging research on Alzheimer and Parkinson diseases.
\end{Insight}

\begin{figure}[H]
    \centering
    \includegraphics[trim=3em 3em 5em 7em, clip, width=\linewidth]{figures/glioma_datasets.pdf}
    \vspace{-2em}
    \caption{Total sequences and citations for each glioma dataset}
    \label{fig:dataset_glioma}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[trim=3em 3em 5em 7em, clip, width=\linewidth]{figures/gbm_datasets.pdf}
    \vspace{-2em}
    \caption{Total sequences and citations for each GBM dataset}
    \label{fig:dataset_gbm}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[trim=3em 3em 5em 7em, clip, width=\linewidth]{figures/metastasis_datasets.pdf}
    \vspace{-2em}
    \caption{Total sequences and citations for each metastasis dataset}
    \label{fig:dataset_metastasis}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[trim=3em 3em 5em 7em, clip, width=\linewidth]{figures/alzheimer_datasets.pdf}
    \vspace{-2em}
    \caption{Total sequences and citations for each Alzheimer dataset}
    \label{fig:dataset_alzheimer}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[trim=3em 3em 5em 7em, clip, width=\linewidth]{figures/parkinson_datasets.pdf}
    \vspace{-2em}
    \caption{Total sequences and citations for each Parkinson dataset}
    \label{fig:dataset_parkinson}
\end{figure}




